Investigating LLM Applications in E-Commerce

The emergence of Large Language Models (LLMs) has revolutionized natural language processing in various applications especially in e-commerce. One crucial step before the application of such LLMs in these fields is to understand and compare the performance in different use cases in such tasks. This paper explored the efficacy of LLMs in the e-commerce domain, focusing on instruction-tuning an open source LLM model with public e-commerce datasets of varying sizes and comparing the performance with the conventional models prevalent in industrial applications. We conducted a comprehensive comparison between LLMs and traditional pre-trained language models across specific tasks intrinsic to the e-commerce domain, namely classification, generation, summarization, and named entity recognition (NER). Furthermore, we examined the effectiveness of the current niche industrial application of very large LLM, using in-context learning, in e-commerce specific tasks. Our findings indicate that few-shot inference with very large LLMs often does not outperform fine-tuning smaller pre-trained models, underscoring the importance of task-specific model optimization.Additionally, we investigated different training methodologies such as single-task training, mixed-task training, and LoRA merging both within domain/tasks and between different tasks. Through rigorous experimentation and analysis, this paper offers valuable insights into the potential effectiveness of LLMs to advance natural language processing capabilities within the e-commerce industry.

==> tab/tab_class.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[h!]
% \small

% \centering

% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%      & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{BERT} \\ \midrule
%      & Micro-F1    & Macro-F1    & Micro-F1      & Macro-F1      \\ \midrule
% 1k   & 0.334       & 0.208       & 0.334         & 0.208         \\
% 5k   & 0.355       & 0.244       & 0.355         & 0.244         \\
% 10k  & 0.397       & 0.213       & 0.397         & 0.213         \\
% 50k  & 0.628       & 0.294       & 0.628         & 0.294         \\
% 100k & 0.658       & 0.147       & 0.658         & 0.147         \\ \bottomrule
% \end{tabular}
% \caption{Comparison of Llama2-7b SFT with finetune BERT on ESCI task 2 dataset.}
% \label{tab:ESCI}
% \end{table}

\begin{table}[tbh!]
\scriptsize

\centering

\begin{tabular}{@{}c|cc|cc|c|cc|cc@{}}
\toprule
 \multicolumn{5}{c}{ESCI Classification} & \multicolumn{5}{c}{QueryNER} \\

\midrule
     & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c|}{BERT}  & & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{BERT} \\ \midrule
  & Micro    & Macro    & Micro      & Macro  &  & Micro    & Macro    & Micro    & Macro       \\
     & F1    & F1    & F1      & F1  &  & F1    & F1    & F1    & F1       \\ \midrule
5k   & \textbf{0.355}       & \textbf{0.244}       & 0.348         & 0.181      & 1k & 0.280        & 0.156        & \textbf{0.539}        & \textbf{0.390} \\
10k  & \textbf{0.397}       & \textbf{0.213}       & 0.379         & 0.192      &     5k & 0.553        & 0.398        & \textbf{0.580}       & \textbf{0.508}  \\
50k  & 0.628       & 0.294      & \textbf{0.629}         & \textbf{0.368}     & 8k & \textbf{0.626}        & \textbf{0.579}        & 0.603        & 0.569        \\
\midrule
Mixtral  & 0.571       & 0.199      &          &      &   & 0.145        & 0.0632        &         &         \\
0-shot  &        &       &          &      &  &         &         &         &         \\
Mixtral  & 0.537       & 0.009      &          &      &   &  0.484        & 0.336        &         &         \\
3-shot  &        &       &          &      &  &         &         &         &         \\
\bottomrule

\end{tabular}
\caption{Comparison of Llama2-7b SFT (LLM) with finetune BERT and Mixtral 8 x 22b zero-shot on ESCI task 2 dataset and QueryNER dataset.}
%\label{tab:ESCI-queryNER}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[h!]
% \small

% \centering

% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%    & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{BERT} \\ \midrule
%    & Micro-F1    & Macro-F1    & Micro-F1    & Macro-F1   \\ \midrule
% % TODO: Ruixiang do we have further decimal place for LLM here?
% 1k & 0.28        & 0.15        & \textbf{0.539}        & \textbf{0.390}     \\
% 5k & 0.55        & 0.39        & \textbf{0.580}       & \textbf{0.508}     \\
% 8k & \textbf{0.62}        & \textbf{0.58}        & 0.603        & 0.569      \\ \bottomrule
% \end{tabular}
% \caption{Comparison of Llama2-7b SFT with finetune BERT on Query NER dataset.}
% \label{tab:ner}
% \end{table}

==> tab/tab_esci_results.tex <==
\begin{table}[tbh!]
\small
\begin{tabular}{@{}lrrll@{}}
\toprule
\multicolumn{5}{c}{ESCI Classification}                                                                                              \\ \midrule
               & \multicolumn{2}{c}{LLM}                                     & \multicolumn{2}{c}{BERT}                              \\ \cmidrule(l){2-5} 
               & \multicolumn{1}{l}{Micro F1} & \multicolumn{1}{l}{Macro F1} & Micro F1                  & Macro F1                  \\ \midrule
5k             & \textbf{0.355}                        & \textbf{0.244}                        & \multicolumn{1}{r}{0.348} & \multicolumn{1}{r}{0.181} \\
10k            & 0.397                        & 0.213                        & \multicolumn{1}{r}{\textbf{0.628}} & \multicolumn{1}{r}{\textbf{0.294}} \\
50k            & 0.628                        & 0.294                        & \multicolumn{1}{r}{\textbf{0.629}} & \multicolumn{1}{r}{\textbf{0.368}} \\ \midrule
Mixtral 0-shot & 0.571                        & 0.199                        &                           &                           \\
Mixtral 3-shot & 0.537                        & 0.009                        &                           &                           \\ \bottomrule
\end{tabular}
\caption{Comparison of Llama2-7b SFT  with finetuned BERT and Mixtral 8 x 22b zero-shot and few-shot on ESCI task 2 dataset.}
\label{tab:ESCI-results}
\end{table}


% \begin{table}[]
% \begin{tabular}{@{}lrr@{}}
% \toprule
% \multicolumn{3}{c}{ESCI Classification}                                      \\ \midrule
%                & \multicolumn{1}{c}{Micro F1} & \multicolumn{1}{c}{Macro F1} \\ \midrule
% BERT 5k        & 0.348                        & 0.181                        \\
% BERT 10k       & 0.628                        & 0.294                        \\
% BERT 50k       & 0.629                        & 0.368                        \\
% Llama2 5k         & 0.355                        & 0.244                        \\
% Llama2 10k        & 0.397                        & 0.213                        \\
% Llama2 50k        & 0.628                        & 0.294                        \\
% Mixtral 0 shot & 0.571                        & 0.199                        \\
% Mixtral 3-shot & 0.537                        & 0.009                        \\ \bottomrule
% \end{tabular}
% \caption{Comparison of Llama2-7b SFT  with finetuned BERT and Mixtral 8 x 22b zero-shot and few-shot on ESCI task 2 dataset.}
% \label{tab:ESCI-results}
% \end{table}

==> tab/tab_ner.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[h!]
% \small

% \centering

% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%    & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{BERT} \\ \midrule
%    & Micro-F1    & Macro-F1    & Micro-F1    & Macro-F1   \\ \midrule
% % TODO: Ruixiang do we have further decimal place for LLM here?
% 1k & 0.28        & 0.15        & \textbf{0.539}        & \textbf{0.390}     \\
% 5k & 0.55        & 0.39        & \textbf{0.580}       & \textbf{0.508}     \\
% 8k & \textbf{0.62}        & \textbf{0.58}        & 0.603        & 0.569      \\ \bottomrule
% \end{tabular}
% \caption{Comparison of Llama2-7b SFT with finetune BERT on Query NER dataset.}
% \label{tab:ner}
% \end{table}


\begin{table}[tbh!]
\small
\begin{tabular}{@{}lrrll@{}}
\toprule
\multicolumn{5}{c}{QueryNER}                                                                                                                           \\ \midrule
               & \multicolumn{2}{c}{LLM}                                     & \multicolumn{2}{c}{BERT}                                                \\ \cmidrule(l){2-5} 
               & \multicolumn{1}{l}{Micro F1} & \multicolumn{1}{l}{Macro F1} & Micro F1                           & Macro F1                           \\ \midrule
5k             & 0.28                         & 0.156                        & \multicolumn{1}{r}{\textbf{0.539}} & \multicolumn{1}{r}{\textbf{0.39}}  \\
10k            & 0.553                        & 0.398                        & \multicolumn{1}{r}{\textbf{0.58}}  & \multicolumn{1}{r}{\textbf{0.508}} \\
50k            & \textbf{0.626}               & \textbf{0.579}               & \multicolumn{1}{r}{0.603}          & \multicolumn{1}{r}{0.569}          \\ \midrule
Mixtral 0-shot & 0.145                        & 0.063                        &                                    &                                    \\
Mixtral 3-shot & 0.484                        & 0.336                        &                                    &                                    \\ \bottomrule
\end{tabular}
\caption{Comparison of Llama2-7b SFT with finetuned BERT and Mixtral 8 x 22b zero-shot and few-shot inference on Query NER dataset.}
\label{tab:ner}
\end{table}

==> tab/tab_summ_gen.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[h!]
% \footnotesize
% \caption{Comparison of Llama2-7b SFT with fine-tune T5 on Review
% Summarization dataset and Product
% Description Generation dataset.}
% \centering
% \label{tab:sum}
% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%     & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{T5}   \\ \midrule
%     & Rouge-1  & Rouge-L & Rouge-1 & Rouge-L \\ \midrule
% 1k  & 0.158           & 0.147  & 0.155   & 0.137            \\
% 5k  & 0.182           & 0.161  & 0.162   & 0.147           \\
% 10k & 0.186           & 0.162  & 0.163   & 0.150            \\
% 25k & 0.187           & 0.165  & 0.169   & 0.158           \\ \bottomrule
% \end{tabular}
% \end{table}



% \begin{tabular}{@{}c|cc|cc@{}}
% \toprule
%     & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{T5}   \\ \midrule
%     & Rouge-1  & Rouge-L & Rouge-1 & Rouge-L \\ \midrule
% 1k  & 0.262          & 0.244   & 0.239        & 0.216   \\
% 5k  & 0.249           & 0.232   & 0.241        & 0.223   \\
% 10k & 0.258          & 0.241   & 0.238         & 0.221  \\
% 25k & 0.237         & 0.222   & 0.232         & 0.215   \\ \bottomrule


\begin{table}[tbh!]
\small
\centering

\begin{tabular}{@{}c|cc|cc|cc|cc@{}}
\toprule
\multicolumn{5}{c|}{Review } & \multicolumn{4}{c}{Desc.}   \\
\multicolumn{5}{c|}{Summarization} & \multicolumn{4}{c}{Generation}   \\
\midrule
    & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c|}{T5} & \multicolumn{2}{c|}{LLM} & \multicolumn{2}{c}{T5}   \\ \midrule
    & R1  & RL & R1 & RL &  R1  & RL & R1 & RL\\ \midrule
1k  & \textbf{0.158} & \textbf{0.147}  & 0.155   & 0.137              & \textbf{0.262}          & \textbf{0.244}   & 0.239        & 0.216 \\
5k  & \textbf{0.182}          & \textbf{0.161}  & 0.162   & 0.147            & \textbf{0.249}        & \textbf{0.232}   & 0.241        & 0.223 \\
10k & \textbf{0.186}         & \textbf{0.162}  & 0.163   & 0.150   & \textbf{0.258}   & \textbf{0.241}   & 0.238  & 0.221\\
25k & \textbf{0.187}  & \textbf{0.165}  & 0.169   & 0.158    & \textbf{0.237}         & \textbf{0.222}   & 0.232         & 0.215\\ 
\midrule 

0-shot & 0.099  & 0.0895  &    &     &        0.248  & 0.229 &          & \\

3-shot & 0.144  & 0.131  &    &     &        0.274  & 0.254 &          & \\ 
 
\bottomrule
\end{tabular}
\caption{Comparison of Llama2-7b SFT (LLM) with fine-tune T5 and zero-shot Mixtral 8 x 22b on Review Summarization dataset and Product
Description Generation dataset.}
%\label{tab:sum}
\end{table}
